Siamese Vision Transformers are Scalable Audio-visual Learners

Traditional audio-visual methods rely on independent audio and visual backbones, which is costly and not scalable. In this work, we investigate using an audio-visual siamese network (AVSiam) for efficient and scalable audio-visual pretraining. Our framework uses a single shared vision transformer backbone to process audio and visual inputs, improving its parameter efficiency, reducing the GPU memory footprint, and allowing us to scale our method to larger datasets and model sizes. We pretrain our model using a contrastive audio-visual matching objective with a multi-ratio random masking scheme, which enables our model to process larger audio-visual instance batches, helpful for contrastive learning. Unlike prior audio-visual methods, our method can robustly handle audio, visual, and audio-visual inputs with a single shared ViT backbone. Furthermore, despite using the shared backbone for both modalities, AVSiam achieves competitive or even better results than prior methods on AudioSet and VGGSound for audio-visual classification and retrieval. Our code is available at https://github.com/GenjiB/AVSiam

==> figure/multi-ratio.tex <==
% \begin{figure*}[t!]
%     \centering
% 	\includegraphics[width=0.50\linewidth]{figure/multi_ratio.pdf}
% \caption{
%     \textbf{Multi-Ratio Masking Scheme.} We apply random masking to both audio and visual tokens in various proportions during each training iteration. 
%     % 
%     Compared to fixed-ratio masking, our multi-ratio random masking scheme enables the model to learn more robust representations by learning from a varying number of tokens while still maintaining high efficiency. 
%     % \gbb{can you include 1 sentence why this is better compared to fixed masking ratio? Also, can you eliminate the the white-space issue caused by "Iteration" hanging at the bottom right?}
%     %
%     % \textbf{Right:} The multi-ratio masking scheme employs random masking of audio and visual tokens at various ratios.
%     %
% }
%     \vspace{\figmargin}
% 	\label{fig:multi_ratio}
% \end{figure*}
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{figure/multi_ratio.pdf}
    \caption{
        \textbf{Multi-Ratio Masking Scheme.} We apply random masking to both audio and visual tokens in various proportions during each training iteration. \ybc{shorten caps}
        % Compared to fixed-ratio masking, our multi-ratio random masking scheme enables the model to learn more robust representations by learning from a varying number of tokens while still maintaining high efficiency.
    }
    \label{fig:multi_ratio}
    \vspace{-10mm}
\end{wrapfigure}

==> rebuttal/inference.tex <==


\begin{table}[t]
\footnotesize
    \caption{
    \textbf{Throughput Comparison.}
    We compare the throughput of our \lav with the state-of-the-art CMBS approach. The throughput is measured using the number of samples per second. In addition to achieving higher accuracy, our method is almost 2$\times$ faster than CMBS.}
    
    \label{tab:flops}
    \centering
    %\footnotesize
    \resizebox{0.45\textwidth}{!}{
    \begin{tabular}{l cccc}
        \toprule
        {Method}  &\makecell{Visual \\Encoder}&\makecell{Audio \\Encoder} & \makecell{ Samples \\  per Sec. $\uparrow$} & \makecell{ Acc $\uparrow$ }  \\  
        \midrule
        %CMBS  [79]     &RN-152\cyansnow&VGGish \cyansnow                 & $1.25$ &  $79.7$ \\
        CMBS~\cite{cvpr22_ave_cmbs}     &Swin-L\cyansnow&VGGish\cyansnow                 & 0.72 &  80.4 \\
        % MBT*  [55]     &ViT-B-16\redfire &AST [20]\redfire                & 2.25 &  $77.8$ \\
        % MBT*  [55]     &ViT-L-16\redfire &AST [20]\redfire                & N/A &  OOM \\
        LAVISH         &\multicolumn{2}{c}{Swin-L\cyansnow~(shared)}  & \bf 1.40 &    \bf 81.1  \\
        \bottomrule
        
    \end{tabular}
    }
\end{table}

==> setup/graphicspath.tex <==
\graphicspath{{figure}, {images}, {example}}


==> setup/symbols.tex <==
% Define math symbols that appear in the texts

\def\xi{\mathbf{x}_i}
\def\yi{\mathbf{y}_i}
